Learning High-level Semantic-Relational Concepts for SLAM

Recent works on SLAM extend their pose graphs with higher-level semantic concepts like Rooms exploiting relationships between them, to provide, not only a richer representation of the situation/environment but also to improve the accuracy of its estimation. Concretely, our previous work, Situational Graphs (S-Graphs+), a pioneer in jointly leveraging semantic relationships in the factor optimization process, relies on semantic entities such as Planes and Rooms, whose relationship is mathematically defined. Nevertheless, there is no unique approach to finding all the hidden patterns in lower-level factor-graphs that correspond to high-level concepts of different natures. It is currently tackled with ad-hoc algorithms, which limits its graph expressiveness. To overcome this limitation, in this work, we propose an algorithm based on Graph Neural Networks for learning high-level semantic-relational concepts that can be inferred from the low-level factor graph. Given a set of mapped Planes our algorithm is capable of inferring Room entities relating to the Planes. Additionally, to demonstrate the versatility of our method, our algorithm can infer an additional semantic-relational concept, i.e. Wall, and its relationship with its Planes. We validate our method in both simulated and real datasets demonstrating improved performance over two baseline approaches. Furthermore, we integrate our method into the S-Graphs+ algorithm providing improved pose and map accuracy compared to the baseline while further enhancing the scene representation.

==> problem_statement.tex <==
\section{Problem Statement and Methodology}
\label{problem_statement}

We aim to define new \textit{room} and \textit{wall} nodes from a set of \textit{wall surface} nodes defined as 2D finite lines.

The solution proposed is inspired in~\cite{sgf}. In the preliminary approach, no edges embedding is used, and the initial nodes embeddings, $v^0_{i}$ are defined as $[c_i, length_{i}, n_{i}]$ where $c_i$ is the centroid of $i_{th}$ node and  $n_{i}$, the normal from the observed side. As a final approach, $v_{i}$ is defined as $[length_{i}, n_{i}]$ and initial edge embedding, $e^0_{ij}$ as, $[c_{j} - c{i}, cd_{ij},n_{j}-n_{i}]$ where $cd_{ij}$ is the closest distance. The embeddings are updated through the GNN iterations following Eq.~\ref{eq:GAT_v} and Eq.~\ref{eq:GAT_e}. Where $g_{v}(·)$ and $g_{e}(·)$ are multi-layer perceptrons, {N}(i) are the neighbors of $i_{th}$ node and $NN(·)$ is SAGEConv for the preliminary approach and Feature-wise Attention for the final approach.
%
\begin{gather}
v_{i}^{l+1} = g_{v} ([v_{i}^l, \max_{j\in\mathcal{N}(i)}(NN(v_i^l,e_{ij}^l,v_j^l))]
\label{eq:GAT_v}
\\
e_{ij}^{l+1} = g_{e}([v_i^l,e_{ij}^l,v_j^l])
\label{eq:GAT_e}
\end{gather}
%
As no prior graph structure can be leveraged, new edges are artificially created in the message-passing graph by node proximity. Ground truth edges contain node relations indicating nodes that belong to the same \textit{room} or \textit{wall}, label the message-passing graph for the training of GNN convolutions which update the embeddings of nodes and edges. After the GNN convolutions, the edge embeddings in the last layer are passed to a linear layer to classify if each edge corresponds to one of the desired relations. Subsequently, the set of predicted relations is used to cluster nodes into \textit{rooms\textit} and \textit{walls} by chained edges of the same type. Once clustered, new \textit{room} and \textit{wall} nodes and \textit{belong to same room} or \textit{belong to same wall} edges are generated. Their features are obtained by employing the same GNN architecture as in Eq.~\ref{eq:GAT_e} to generate new embeddings. Finally, the node embeddings from Eq.~\ref{eq:GAT_v} are fed to a linear layer to fit the node feature dimension.

